New Faithfulness-Centric Interpretability Paradigms for Natural Language Processing

As machine learning becomes more widespread and is used in more critical applications, it's important to provide explanations for these models, to prevent unintended behavior. Unfortunately, many current interpretability methods struggle with faithfulness. Therefore, this Ph.D. thesis investigates the question "How to provide and ensure faithful explanations for complex general-purpose neural NLP models?" The main thesis is that we should develop new paradigms in interpretability. This is achieved by first developing solid faithfulness metrics and then applying the lessons learned from this investigation to develop new paradigms. The two new paradigms explored are faithfulness measurable models (FMMs) and self-explanations. The idea in self-explanations is to have large language models explain themselves, we identify that current models are not capable of doing this consistently. However, we suggest how this could be achieved. The idea of FMMs is to create models that are designed such that measuring faithfulness is cheap and precise. This makes it possible to optimize an explanation towards maximum faithfulness, which makes FMMs designed to be explained. We find that FMMs yield explanations that are near theoretical optimal in terms of faithfulness. Overall, from all investigations of faithfulness, results show that post-hoc and intrinsic explanations are by default model and task-dependent. However, this was not the case when using FMMs, even with the same post-hoc explanation methods. This shows, that even simple modifications to the model, such as randomly masking the training dataset, as was done in FMMs, can drastically change the situation and result in consistently faithful explanations. This answers the question of how to provide and ensure faithful explanations.

==> chapters/2-literature-review/content/motivation.tex <==
\section{Motivations for interpretability}
\label{sec:survey:motivation-for-interpretability}

The need for interpretability comes primarily from an ``incompleteness in the problem formalization'' \citep{Doshi-Velez2017a}, meaning if the model was constrained and optimized to prevent all possible ethical issues, interpretability would be much less relevant. However, because perfect optimization is unlikely, hence \motivation{safety} and \motivation{ethics} are strong motivations for interpretability.

Additionally, when models misbehave, there is a need for explanations to hold people or companies accountable; hence, \motivation{acountability} is often a core motivation for interpretability. Finally, explanations are often useful, or sometimes necessary, for gaining \motivation{scientific understanding} about models. This section aims to elaborate on what exactly is understood by these terms and how interpretability can address them.

% TODO: how could this be written without assuming what ``common ethical and moral'' is?
\paragraph{Ethics,} in the context of interpretability, is about ensuring that the model's behavior is aligned with common ethical and moral values. Because there does not exist an exact measure for this desideratum, this is ultimately something that should be judged qualitatively by humans, for example, by an \emph{ethics review committee}, who will inspect the model explanations.

For some ethical concerns, such as discrimination, it may be possible to measure and satisfy this ethical concern via fairness metrics and debiasing techniques \citep{Garrido-Munoz2021}. However, this often requires a finite list of protected attributes \citep{Ho2021}, and such a list will likely be incomplete, hence the need for a qualitative assessment \citep{Doshi-Velez2017a, Lipton2018}.

\paragraph{Safety,} is about ensuring the model performs within expectations in deployment. As it is nearly impossible to truly test the model in the end-to-end context that it will be deployed, ensuring \motivation{safety} does to some extent involve qualitative assessment \citep{Doshi-Velez2017a}. \citet{Lipton2018} frames this as \motivation{trust}, and suggests one interpretation of this is ``that we feel comfortable relinquishing control to it''.

While all types of interpretability can help with \motivation{safety}, in particular, \type{sec:survey:adversarial-examples}{adversarial examples} and \type{sec:survey:counterfactuals}{counterfactuals} are useful, as they evaluate the model on data outside the test distribution. \citet{Lipton2018} frames this in the broader context of \motivation{transferability}, which is the model's robustness to adversarial attacks and distributional shifts.

\paragraph{Accountability,} relates to explaining the model when it does fail in production. The ``right to explanation'', regarding the logic involved in the model's prediction, is increasingly being adopted, most notably in the EU via its GDPR legislation. However, the US and UK have also expressed support for such regulation \citep{Doshi-Velez2017}. Additionally, industries, such as banking, are already required to audit their models \citep{Bhatt2020}.

\motivation{Accountability} is perhaps the core motivation of interpretability, as \citet{Miller2019} writes, ``Interpretability is the degree to which a human can understand the cause of a decision'', and it is exactly the causal reasoning that is relevant in \motivation{accountability} \citep{Doshi-Velez2017}. 

\paragraph{Scientific Understanding,} addresses a need from researchers and scientists to generate hypotheses and knowledge. As \citet{Doshi-Velez2017a} frames it, sometimes the best way to start such a process is to ask for explanations. In model development, explanations can also be useful for \motivation{model debugging} \citep{Bhatt2020}, which is often facilitated by the same kinds of explanations.


==> chapters/3-recursive-roar/table/datasets.tex <==
\begin{tabular}{lccc} 
\toprule   
Dataset & Sequence & \multicolumn{2}{c}{Performance [\%]} \\
\cmidrule(r){3-4}
& length & LSTM & RoBERTa \\
\midrule   
Anemia & 2267 & $88^{+1.1}_{-2.2}$ & $86^{+0.6}_{-0.7}$ \\
Diabetes & 2207 & $81^{+2.2}_{-2.9}$ & $76^{+0.7}_{-0.6}$ \\
IMDB & 181 & $90^{+0.4}_{-0.7}$ & $95^{+0.2}_{-0.2}$ \\
SNLI & 16 & $78^{+0.2}_{-0.3}$ & $91^{+0.1}_{-0.1}$ \\
SST & 20 & $82^{+0.6}_{-1.0}$ & $94^{+0.3}_{-0.3}$ \\
bAbI-1 & 38 & $100^{+0.0}_{-0.1}$ & $100^{+0.0}_{-0.0}$ \\
bAbI-2 & 96 &  $68^{+9.1}_{-19.1}$ & $100^{+0.1}_{-0.1}$ \\
bAbI-3 & 308 & $60^{+6.5}_{-4.9}$ & $81^{+6.8}_{-20.0}$ \\
\bottomrule
\end{tabular}


==> chapters/3-recursive-roar/table/riemann_samples.tex <==
\begin{tabular}{llllrrrrr}
\toprule
       &     &              & {} & \multicolumn{5}{l}{rank-error} \\
       &     &              & ranks &        all &       c-1 &      c-10 &      q-10 &      q-90 \\
dataset & samples & walltime & abs_error &            &           &           &           &           \\
\midrule
\multirow{12}{*}{Anemia} & 2   & 101.245534   & 4.212499e-04 &   0.981569 &  0.359217 &  0.670127 &  0.931639 &  0.985561 \\
       & 5   & 224.211633   & 1.900731e-04 &   0.952694 &  0.223809 &  0.486668 &  0.854859 &  0.962467 \\
       & 10  & 465.211974   & 9.743480e-05 &   0.910150 &  0.165410 &  0.361784 &  0.763002 &  0.926461 \\
       & 20  & 855.312985   & 4.272683e-05 &   0.822572 &  0.085673 &  0.223873 &  0.594393 &  0.846262 \\
       & 30  & 1288.854942  & 2.567901e-05 &   0.732999 &  0.060966 &  0.158623 &  0.469494 &  0.759835 \\
       & 40  & 1917.144134  & 1.705118e-05 &   0.639946 &  0.044120 &  0.118931 &  0.370341 &  0.666477 \\
       & 50  & 2416.830668  & 1.156951e-05 &   0.543600 &  0.032087 &  0.088545 &  0.285903 &  0.567741 \\
       & 60  & 2808.785240  & 8.211632e-06 &   0.448582 &  0.030002 &  0.076207 &  0.224991 &  0.469050 \\
       & 70  & 2816.397905  & 5.715537e-06 &   0.350925 &  0.023584 &  0.063084 &  0.170533 &  0.366898 \\
       & 80  & 3215.318586  & 3.986991e-06 &   0.253103 &  0.021980 &  0.057292 &  0.127318 &  0.264332 \\
       & 90  & 3450.266509  & 2.162507e-06 &   0.146725 &  0.016044 &  0.041778 &  0.079742 &  0.152731 \\
       & 100 & 4290.197410  & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{Diabetes} & 2   & 216.577702   & 3.693328e-04 &   0.987038 &  0.039321 &  0.414004 &  0.932146 &  0.987547 \\
       & 5   & 493.015442   & 1.226521e-04 &   0.969338 &  0.019529 &  0.265596 &  0.883182 &  0.970705 \\
       & 10  & 1044.036231  & 5.613671e-05 &   0.939109 &  0.011348 &  0.161049 &  0.811889 &  0.941372 \\
       & 20  & 2131.249034  & 2.473134e-05 &   0.876072 &  0.006422 &  0.085125 &  0.690026 &  0.879103 \\
       & 30  & 3037.823552  & 1.438819e-05 &   0.808189 &  0.004662 &  0.054249 &  0.582591 &  0.811228 \\
       & 40  & 4094.933739  & 9.237436e-06 &   0.735016 &  0.003519 &  0.036348 &  0.484113 &  0.737431 \\
       & 50  & 5792.294085  & 6.153519e-06 &   0.655240 &  0.003167 &  0.025255 &  0.393797 &  0.656560 \\
       & 60  & 6408.906722  & 4.100251e-06 &   0.567722 &  0.002903 &  0.018174 &  0.309460 &  0.567615 \\
       & 70  & 6668.413624  & 2.634924e-06 &   0.469620 &  0.002375 &  0.012201 &  0.229474 &  0.467858 \\
       & 80  & 7265.292086  & 1.536612e-06 &   0.356380 &  0.002199 &  0.007855 &  0.152747 &  0.352923 \\
       & 90  & 9419.508060  & 6.827888e-07 &   0.216496 &  0.001319 &  0.004601 &  0.077924 &  0.212074 \\
       & 100 & 10339.881488 & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{IMDB} & 2   & 43.092894    & 1.037579e-02 &   0.871993 &  0.085208 &  0.391808 &  0.499771 &  0.866614 \\
       & 5   & 89.239690    & 4.029346e-03 &   0.744075 &  0.035474 &  0.207157 &  0.302828 &  0.735468 \\
       & 10  & 171.989350   & 1.917285e-03 &   0.587424 &  0.017389 &  0.110913 &  0.177513 &  0.576848 \\
       & 20  & 330.252559   & 8.541130e-04 &   0.390915 &  0.007806 &  0.053173 &  0.089459 &  0.380840 \\
       & 30  & 475.414340   & 4.986248e-04 &   0.273621 &  0.004367 &  0.031417 &  0.054708 &  0.265358 \\
       & 40  & 635.290816   & 3.206723e-04 &   0.195633 &  0.002782 &  0.020326 &  0.035992 &  0.189241 \\
       & 50  & 841.868045   & 2.138323e-04 &   0.139993 &  0.001778 &  0.013224 &  0.024141 &  0.135105 \\
       & 60  & 985.008599   & 1.425776e-04 &   0.098242 &  0.001237 &  0.008811 &  0.016144 &  0.094659 \\
       & 70  & 1141.382244  & 9.166776e-05 &   0.065693 &  0.000657 &  0.005750 &  0.010543 &  0.063223 \\
       & 80  & 1284.326926  & 5.347724e-05 &   0.039502 &  0.000232 &  0.003215 &  0.006170 &  0.037963 \\
       & 90  & 1467.748873  & 2.376944e-05 &   0.017988 &  0.000077 &  0.001465 &  0.002712 &  0.017278 \\
       & 100 & 1628.388538  & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{SNLI} & 2   & 128.844450   & 3.029601e-02 &   0.678536 &  0.206067 &  0.630414 &  0.235966 &  0.676351 \\
       & 5   & 201.026176   & 9.867780e-03 &   0.409434 &  0.076203 &  0.354065 &  0.092569 &  0.407639 \\
       & 10  & 310.218702   & 4.700520e-03 &   0.251190 &  0.036740 &  0.206646 &  0.045774 &  0.249090 \\
       & 20  & 541.730724   & 2.104439e-03 &   0.132711 &  0.016549 &  0.104526 &  0.020897 &  0.130988 \\
       & 30  & 799.702943   & 1.230916e-03 &   0.082936 &  0.009623 &  0.064042 &  0.012232 &  0.081641 \\
       & 40  & 1138.658037  & 7.923950e-04 &   0.055321 &  0.006170 &  0.042151 &  0.007891 &  0.054385 \\
       & 50  & 1382.009402  & 5.287155e-04 &   0.037886 &  0.004151 &  0.028631 &  0.005320 &  0.037201 \\
       & 60  & 1497.165611  & 3.526816e-04 &   0.025691 &  0.002752 &  0.019303 &  0.003556 &  0.025202 \\
       & 70  & 1719.830389  & 2.268183e-04 &   0.016698 &  0.001698 &  0.012468 &  0.002208 &  0.016348 \\
       & 80  & 2233.465927  & 1.323520e-04 &   0.009890 &  0.000984 &  0.007363 &  0.001277 &  0.009679 \\
       & 90  & 2445.198340  & 5.883791e-05 &   0.004465 &  0.000446 &  0.003319 &  0.000570 &  0.004380 \\
       & 100 & 2595.697045  & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{SST} & 2   & 6.179342     & 4.125003e-02 &   0.345318 &  0.063566 &  0.273893 &  0.097015 &  0.346495 \\
       & 5   & 10.537298    & 1.616349e-02 &   0.171881 &  0.026513 &  0.126903 &  0.041160 &  0.172109 \\
       & 10  & 11.270489    & 7.688394e-03 &   0.090985 &  0.012387 &  0.063882 &  0.019260 &  0.090847 \\
       & 20  & 14.584255    & 3.424350e-03 &   0.043213 &  0.005868 &  0.029249 &  0.009417 &  0.042925 \\
       & 30  & 19.207759    & 1.998944e-03 &   0.025854 &  0.003151 &  0.016976 &  0.005053 &  0.025529 \\
       & 40  & 23.707140    & 1.285492e-03 &   0.016397 &  0.002391 &  0.010675 &  0.003405 &  0.016165 \\
       & 50  & 27.695689    & 8.571772e-04 &   0.011072 &  0.001630 &  0.007465 &  0.002427 &  0.011019 \\
       & 60  & 33.658953    & 5.715312e-04 &   0.007224 &  0.001087 &  0.004852 &  0.001612 &  0.007185 \\
       & 70  & 38.382564    & 3.674495e-04 &   0.004556 &  0.000543 &  0.003181 &  0.000851 &  0.004546 \\
       & 80  & 40.515218    & 2.143618e-04 &   0.002636 &  0.000435 &  0.001813 &  0.000525 &  0.002616 \\
       & 90  & 48.007606    & 9.527827e-05 &   0.001150 &  0.000217 &  0.000788 &  0.000290 &  0.001149 \\
       & 100 & 48.787989    & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{bAbI-1} & 2   & 7.425629     & 1.081415e-01 &   0.851283 &  0.249364 &  0.718864 &  0.453836 &  0.847859 \\
       & 5   & 8.124638     & 3.858272e-02 &   0.690323 &  0.163909 &  0.503700 &  0.307677 &  0.684464 \\
       & 10  & 10.991558    & 1.176209e-02 &   0.450357 &  0.063091 &  0.254918 &  0.148500 &  0.442510 \\
       & 20  & 13.864422    & 2.284346e-03 &   0.203838 &  0.013818 &  0.080291 &  0.042392 &  0.197764 \\
       & 30  & 17.867403    & 7.844175e-04 &   0.099069 &  0.005000 &  0.029945 &  0.014994 &  0.094974 \\
       & 40  & 23.031856    & 3.776491e-04 &   0.050868 &  0.002727 &  0.014027 &  0.006545 &  0.048273 \\
       & 50  & 30.729127    & 2.219148e-04 &   0.029322 &  0.001364 &  0.007718 &  0.003698 &  0.027720 \\
       & 60  & 30.525028    & 1.401889e-04 &   0.017799 &  0.000818 &  0.004473 &  0.002283 &  0.016772 \\
       & 70  & 36.853598    & 8.827613e-05 &   0.011075 &  0.000455 &  0.002809 &  0.001252 &  0.010478 \\
       & 80  & 41.546208    & 5.110717e-05 &   0.006300 &  0.000273 &  0.001645 &  0.000945 &  0.005965 \\
       & 90  & 44.202871    & 2.296823e-05 &   0.003196 &  0.000273 &  0.000864 &  0.000521 &  0.003037 \\
       & 100 & 45.209531    & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{bAbI-2} & 2   & 15.312163    & 2.878886e-01 &   0.957670 &  0.535091 &  0.871600 &  0.824966 &  0.956850 \\
       & 5   & 19.680807    & 2.724161e-01 &   0.939688 &  0.437727 &  0.816827 &  0.766893 &  0.938413 \\
       & 10  & 27.398557    & 1.840523e-01 &   0.911351 &  0.343909 &  0.745300 &  0.695440 &  0.909493 \\
       & 20  & 45.474422    & 1.289366e-01 &   0.867509 &  0.265364 &  0.658391 &  0.615779 &  0.865040 \\
       & 30  & 64.054374    & 1.165800e-01 &   0.836549 &  0.239727 &  0.612045 &  0.577744 &  0.833669 \\
       & 40  & 77.930287    & 9.688232e-02 &   0.811348 &  0.211636 &  0.573982 &  0.541338 &  0.808298 \\
       & 50  & 104.210327   & 6.895255e-02 &   0.773628 &  0.146636 &  0.502655 &  0.476521 &  0.769994 \\
       & 60  & 131.502538   & 8.642209e-02 &   0.772235 &  0.191909 &  0.530418 &  0.505219 &  0.769344 \\
       & 70  & 152.124177   & 8.517199e-02 &   0.757961 &  0.189273 &  0.517764 &  0.495242 &  0.754956 \\
       & 80  & 143.654563   & 7.428072e-02 &   0.738748 &  0.175091 &  0.490282 &  0.470681 &  0.735710 \\
       & 90  & 167.494699   & 8.025901e-02 &   0.728735 &  0.177909 &  0.489391 &  0.470783 &  0.726110 \\
       & 100 & 192.393586   & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\cline{1-9}
\multirow{12}{*}{bAbI-3} & 2   & 27.774496    & 1.729354e-01 &   0.982463 &  0.562636 &  0.864336 &  0.913653 &  0.981887 \\
       & 5   & 49.460336    & 1.114488e-01 &   0.970721 &  0.410455 &  0.777245 &  0.855408 &  0.969511 \\
       & 10  & 82.138040    & 8.716298e-02 &   0.949756 &  0.295727 &  0.653200 &  0.774445 &  0.947338 \\
       & 20  & 172.415194   & 7.651677e-02 &   0.915627 &  0.216000 &  0.530645 &  0.685473 &  0.911663 \\
       & 30  & 214.012361   & 9.021264e-02 &   0.893471 &  0.216364 &  0.492391 &  0.647871 &  0.888786 \\
       & 40  & 323.617345   & 7.589681e-02 &   0.874283 &  0.192455 &  0.453400 &  0.614128 &  0.869164 \\
       & 50  & 386.221956   & 4.653517e-02 &   0.849599 &  0.133000 &  0.385218 &  0.559955 &  0.843597 \\
       & 60  & 445.447177   & 2.164273e-01 &   0.846893 &  0.180727 &  0.415809 &  0.575162 &  0.840993 \\
       & 70  & 473.667068   & 8.822861e-02 &   0.838317 &  0.197091 &  0.415827 &  0.569455 &  0.832384 \\
       & 80  & 560.828869   & 6.845812e-02 &   0.825183 &  0.176818 &  0.392682 &  0.548454 &  0.818878 \\
       & 90  & 630.839226   & 8.787030e-01 &   0.819522 &  0.184818 &  0.395764 &  0.548138 &  0.813215 \\
       & 100 & 726.316175   & 0.000000e+00 &   0.000000 &  0.000000 &  0.000000 &  0.000000 &  0.000000 \\
\bottomrule
\end{tabular}


==> chapters/3-recursive-roar/table/sparsity.tex <==
\begin{tabular}{llll}
\toprule
       & {} & \multicolumn{2}{l}{total importance} \\
       & k &                        1  &                         10 \\
dataset & importance measure &                           &                            \\
\midrule
\multirow{3}{*}{Anemia} & Attention &   $1\%^{+1.1\%}_{-0.5\%}$ &    $7\%^{+7.5\%}_{-3.8\%}$ \\
       & Gradient &   $1\%^{+0.2\%}_{-0.2\%}$ &    $6\%^{+1.3\%}_{-1.1\%}$ \\
       & Integrated Gradient &   $2\%^{+0.9\%}_{-0.6\%}$ &   $14\%^{+4.5\%}_{-3.5\%}$ \\
\cline{1-4}
\multirow{3}{*}{Diabetes} & Attention &  $22\%^{+3.6\%}_{-3.2\%}$ &   $53\%^{+5.5\%}_{-5.6\%}$ \\
       & Gradient &   $7\%^{+1.1\%}_{-1.0\%}$ &   $32\%^{+2.7\%}_{-2.6\%}$ \\
       & Integrated Gradient &  $18\%^{+1.6\%}_{-1.5\%}$ &   $43\%^{+3.4\%}_{-3.3\%}$ \\
\cline{1-4}
\multirow{3}{*}{IMDB} & Attention &   $9\%^{+2.2\%}_{-1.8\%}$ &   $43\%^{+9.9\%}_{-9.4\%}$ \\
       & Gradient &   $3\%^{+0.5\%}_{-0.4\%}$ &   $20\%^{+3.1\%}_{-2.7\%}$ \\
       & Integrated Gradient &   $9\%^{+1.1\%}_{-1.0\%}$ &   $39\%^{+2.7\%}_{-2.6\%}$ \\
\cline{1-4}
\multirow{3}{*}{SNLI} & Attention &  $38\%^{+1.3\%}_{-1.3\%}$ &   $95\%^{+0.5\%}_{-0.5\%}$ \\
       & Gradient &  $31\%^{+0.5\%}_{-0.5\%}$ &   $93\%^{+0.3\%}_{-0.3\%}$ \\
       & Integrated Gradient &  $28\%^{+0.9\%}_{-0.9\%}$ &   $91\%^{+0.2\%}_{-0.2\%}$ \\
\cline{1-4}
\multirow{3}{*}{SST} & Attention &  $26\%^{+7.4\%}_{-6.2\%}$ &   $86\%^{+4.9\%}_{-7.0\%}$ \\
       & Gradient &  $11\%^{+1.5\%}_{-1.3\%}$ &   $69\%^{+3.1\%}_{-3.3\%}$ \\
       & Integrated Gradient &  $25\%^{+2.6\%}_{-2.4\%}$ &   $86\%^{+1.0\%}_{-1.0\%}$ \\
\cline{1-4}
\multirow{3}{*}{bAbI-1} & Attention &  $84\%^{+4.8\%}_{-6.3\%}$ &  $100\%^{+0.3\%}_{-0.6\%}$ \\
       & Gradient &  $18\%^{+2.9\%}_{-2.6\%}$ &   $74\%^{+2.1\%}_{-2.3\%}$ \\
       & Integrated Gradient &  $28\%^{+3.4\%}_{-3.1\%}$ &   $85\%^{+3.4\%}_{-4.2\%}$ \\
\cline{1-4}
\multirow{3}{*}{bAbI-2} & Attention &  $74\%^{+4.6\%}_{-5.2\%}$ &   $99\%^{+0.4\%}_{-0.6\%}$ \\
       & Gradient &  $10\%^{+1.9\%}_{-1.6\%}$ &   $48\%^{+3.3\%}_{-3.3\%}$ \\
       & Integrated Gradient &  $12\%^{+1.9\%}_{-1.7\%}$ &   $51\%^{+3.9\%}_{-3.9\%}$ \\
\cline{1-4}
\multirow{3}{*}{bAbI-3} & Attention &  $60\%^{+6.1\%}_{-6.5\%}$ &   $98\%^{+0.7\%}_{-1.0\%}$ \\
       & Gradient &   $6\%^{+0.5\%}_{-0.5\%}$ &   $32\%^{+2.1\%}_{-2.0\%}$ \\
       & Integrated Gradient &   $8\%^{+1.4\%}_{-1.2\%}$ &   $37\%^{+4.1\%}_{-3.9\%}$ \\
\bottomrule
\end{tabular}


==> chapters/4-fmm/tables/manual/importance-measures.tex <==
\begin{tabular}{llll}
\toprule
Category                   & Full name             & Short name   & Variants \\ \midrule
\multirow{3}{*}{Gradient}  & Gradient w.r.t. input & Grad         & absolute \\ 
                           & Input times gradient  & x $\odot$ grad & both \\ 
                           & Integrated gradient   & IG           & both \\  \cmidrule{2-4}
\multirow{2}{*}{Occlusion} & Leave-on-out          & LOO          & both \\
                           & Beam-search           & Beam         & signed \\
\bottomrule
\end{tabular}
